Finding good policies in average-reward Markov Decision Processes without prior knowledge

We revisit the identification of an $\varepsilon$-optimal policy in average-reward Markov Decision Processes (MDP). In such MDPs, two measures of complexity have appeared in the literature: the diameter, $D$, and the optimal bias span, $H$, which satisfy $H\leq D$. Prior work have studied the complexity of $\varepsilon$-optimal policy identification only when a generative model is available. In this case, it is known that there exists an MDP with $D \simeq H$ for which the sample complexity to output an $\varepsilon$-optimal policy is $\Omega(SAD/\varepsilon^2)$ where $S$ and $A$ are the sizes of the state and action spaces. Recently, an algorithm with a sample complexity of order $SAH/\varepsilon^2$ has been proposed, but it requires the knowledge of $H$. We first show that the sample complexity required to estimate $H$ is not bounded by any function of $S,A$ and $H$, ruling out the possibility to easily make the previous algorithm agnostic to $H$. By relying instead on a diameter estimation procedure, we propose the first algorithm for $(\varepsilon,\delta)$-PAC policy identification that does not need any form of prior knowledge on the MDP. Its sample complexity scales in $SAD/\varepsilon^2$ in the regime of small $\varepsilon$, which is near-optimal. In the online setting, our first contribution is a lower bound which implies that a sample complexity polynomial in $H$ cannot be achieved in this setting. Then, we propose an online algorithm with a sample complexity in $SAD^2/\varepsilon^2$, as well as a novel approach based on a data-dependent stopping rule that we believe is promising to further reduce this bound.

==> sectionsN/appmixing.tex <==
% !TeX root = ../neurips_2024.tex

\section{Suboptimality time of MDP $\mathcal{M}_p$}\label{app:mixing}

We propose to prove the following: for any $N$, for any $p<1/N$ and any $p' < \frac{1-\varepsilon}{1+\varepsilon}p$, the policy in full lines $\pi$ is optimal for more than $N$ steps, but is not $\varepsilon$-optimal in average reward.

\begin{figure}[!ht]
	\centering
	\begin{tikzpicture}[node distance={15mm},thick,main/.style = {draw,circle}]
		\node[main] (1) {1};
		\node[main] (2) [left of=1] {2};
		\node[main] (3) [right of=1] {3};
		\draw[->] (1) to [loop above,looseness=15]node{$1,1-p$} (1);
		\draw[->,dashed] (1) to [loop below,looseness=15]node{$0,1-p$} (1);
		\draw[->,dashed] (2) to [loop left,looseness=15]node{$1,1-p'$} (2);
		\draw[->] (3) to [loop right,looseness=15]node{$0,1-p'$} (3);
		\draw[->,dashed] (1) to [out=200,in=-20]node[midway,below]{$0,p$} (2);
		\draw[->,dashed] (2) to [out=20,in=160]node[midway,above]{$1,p'$} (1);
		\draw[->] (1) to [out=20,in=160]node[midway, above, sloped]{$1,p$} (3);
		\draw[->] (3) to [out=200,in=-20]node[midway,below]{$0,p'$} (1);
		%\draw[->] (2) to node[midway, below,sloped]{$0,1$} (1);
		%\draw[->] (3) to node[midway, below,sloped]{$0,1$} (1);
	\end{tikzpicture}
	\repeatcaption{fig:mixing}{MDP $\mathcal{M}_{p,p'}$}
\end{figure}

For that, we define $u_n$ the probability of being in state $1$ at timestep $n$. We note that $u_n$ does not depend on the policy chosen. Since we know $\left\{ \begin{aligned} &u_0=1 \\ &u_{n+1}= p'\end{aligned}\right.$, we have \[u_n= (1-p-p')^n\left(1-\frac{p'}{p+p'}\right) +\frac{p'}{p+p'}\]

Therefore, the (asymptotic) gain for $\pi$ is $g_\pi=\frac{p'}{p+p'}$, while that of the dashed line policy $\pi'$ is $g_{\pi'}=1-\frac{p'}{p+p'}=\frac{p}{p+p'}$. Since $p' < \frac{1-\varepsilon}{1+\varepsilon}p$, \begin{align*}
	%p' &<\frac{1-\varepsilon}{1+\varepsilon}p \\
	p'(1+\varepsilon) &< p(1-\varepsilon)\\
	p' &< p-(p+p')\varepsilon\\
	g_\pi &< g_{\pi'}-\varepsilon
\end{align*}
and we have indeed that $\pi$ is not $\varepsilon$-optimal.

Moreover, the empirical reward up to step $n$ for policy $\pi$ is $r_n=\sum_{t=0}^n u_n$, and $r_n'=n+1-\sum_{t=0}^n u_n$ for policy $\pi'$. As $\left( r_n/n\right)_n$ is decreasing and $\left( r_n'/n\right)_n$ is increasing, policy $\pi'$ becomes better than $\pi$ as long as $\sum_{t=0}^n u_n \leq \frac{n+1}{2}$, that is, as long as \begin{align*}
	(n+1)\frac{p'}{p+p'} + \left(1-\frac{p'}{p+p'}\right)\sum_{t=0}^n(1-p-p')^t &\leq \frac{n+1}{2} \\
	\frac{p}{p+p'} \cdot \frac{1}{n+1}\cdot \frac{1-(1-p-p')^{n+1}}{p+p'}&\leq \frac{1}{2}-\frac{p'}{p+p'}
\end{align*} which is not satisfied \[ \frac{p}{p+p'} \cdot \frac{1}{n+1}\cdot \frac{(n+1)(p+p')-n(n+1)(p+p')^2}{p+p'}\leq \frac{1}{2}-\frac{p'}{p+p'}\] by using that $(1-x)^{n+1} > 1-(n+1)x+n(n+1)x^2/2$ for any $0<x<1$. Finally, we require $\frac{-n}{2}\leq \left(\frac{1}{2}-\frac{p'}{p+p'}\right)\frac{1}{p} -\frac{1}{p+p'}$, ie $n\geq \frac{1}{p}\geq N$.
